Automated Verification of Accountability in Security Protocols

Accountability is a recent paradigm in security protocol design which aims to eliminate traditional trust assumptions on parties and hold them accountable for their misbehavior. It is meant to establish trust in the first place and to recognize and react if this trust is violated. In this work, we discuss a protocol agnostic definition of accountability: a protocol provides accountability (w.r.t. some security property) if it can identify all misbehaving parties, where misbehavior is defined as a deviation from the protocol that causes a security violation. We provide a mechanized method for the verification of accountability and demonstrate its use for verification and attack finding on various examples from the accountability and causality literature, including Certificate Transparency and Kroll Accountable Algorithms protocol. We reach a high degree of automation by expressing accountability in terms of a set of trace properties and show their soundness and completeness.

==> cases-kroll.tex <==
% \subsubsection*{Kroll's Accountable Algorithms protocol} 
\subsection{Kroll's Accountable Algorithms
protocol}\label{sec:cases-kroll}

The protocol lets an authority $A$, e.g., a tax authority, perform
computations for a number of subjects  $S_1$ to $S_n$, e.g., the
validation of tax returns.
%
It derives its name from the feature that any subject can verify,
using a public log, that the value it receives has been computed
correctly w.r.t.\ the input it provides and some secret information
that is the same for all parties.
%
We substantially extend this protocol to also provide accountability
for the subjects: if a subject decides to falsely claim that the
authority cheated, we can validate their claim.
%
This scenario is very instructive, as now any party emitting logs or
claims can just lie. It also 
demonstrates that a central
trusted party is not needed to provide accountability.
It thus goes beyond the previous case studies both in scope and 
in terms of conceptual complexity.

% \input{gfx/accountable-algorithms}

\begin{figure}[!htb]%{{{fig
\centering
 \begin{lstlisting}
S$\defeq$ let res     = <'2', z, rz, rx>
      claim   = <'3', x, z, res, sig_res, rxp>
      Cxp     = commit(x, rxp)
      m1      = <'1', x, rxp, sign(Cxp, sk('S'))>
      sig_cxp = fst(log)
      zkp     = fst(snd(log))
      CxpL    = snd(snd(log))
      Cy      = fst(snd(Pub(zkp)))
  in 
  lookup <'A', 'Init'> as CyL in 
  new x; new rxp; out (<m1, sign(m1,sk('S'))>); 
  lookup <'A','Log','S'> as log in
  if and4( verZK(zkp), eq(sig_cxp,sign(Cxp, sk('S'))),
           eq(CxpL,Cxp), eq(Cy, CyL)) then 
                in (<res, sig_res>); 
                if verify(sig_res, res, pk(sk('A')))=true() then
                  out (<claim, sign(claim, sk('S'))>)

A$\defeq$ let m1 = <'1', x, rxp, sig_cxp>
      z      = f(x, y)
      res    = <'2', z, rz, rx>
      Cx         = commit(x, rx)
      Cy         = commit(y, ry)
      Cz         = commit(z, rz)
      Cxp        = commit(x, rxp)
      zkp        = ZK(<Cx,Cy,Cz>,x,y,z,rx,ry,rz)
      sig_res    = sign(res, sk('A'))
  in
  new y; new ry;
  insert <'A', 'Init'>, Cy;
  in (<m1, sig_m1>); new rx; new rz;
  if and3(verify(sig_m1,m1,pk(sk('S'))), 
      eq(x, open(Cxp,rxp)), 
      verify(sig_cxp,Cxp,pk(sk('S')))) then 
      out (<res, sig_res>);  // send result to S
      insert <'A','Log','S'>, <sig_cxp, zkp, Cxp>;
      insert <'A','Final'>, true()

!($A$ || $S$) || $J$ ||
  out(pk(sk('A'))); out(pk(sk('S')))
||  
 !(in('c',<'corrupt',x>);event Corrupted(x);out('c',sk(x));
   !((if x='A' then in(y); insert <'A','Init'>,y)
    ||(if x='A' then in(y); insert <'A','Log','S'>, y)
    ||(if x='A' then in(y); insert <'A','Final'>, y)) 
    ||(if x='A' then lookup <'A','Log','S'> as y in out(y))
    ||(if x='S' then lookup <'A','Log','S'> as y in out(y))
    ))
 \end{lstlisting}
\caption{Accountable algorithms protocol.}
\label{fig:accountable-algorithms-protocol}
\end{figure} %}}}


The goal is to compute a function $f$ on inputs $x$ and $y$,
$f$ representing an arbitrary algorithm, $x$ the subject's input, and
$y$ some secret policy that $f$ takes into account (e.g., an income threshold
to decide which tax returns need extra scrutiny), but is the same for
all subjects.
%
The authority commits on this value (see Figure~\ref{fig:honest-protocol-run-for-example-ex}).
%
We model commitments using the symbols
$\commit/2$,
$\open/2$, $\verCom/2$ and equations
$\open(\commit(m,r),r)=m$
and
$\verCom(\commit(m,r),r)=\true()$.
%
The subject sends its input $x$ along with randomness for its desired
commitment $r_{x'}$ and a signature for the commitment 
$C_{x'}\defeq \commit(x,r_{x'})$.
%
Now the authority computes $z=f(x,y)$ and returns $z$, as well as
randomness which was used to compute the two commitments $C_x$ on $x$
and $C_z$ on $z$.
%
The signed commitment $C_{x'}$ and a zero-knowledge proof (ZKP) are stored
in the log. 
%
The log is modelled via the store and a global assumption that entries
cannot be overwritten.
%
The ZKP contains the three commitments $C_x$, $C_y$ and
$C_z$ and shows that they are commitments to $x$, $y$ and $z$ such
that $f(x,y)=z$. Using this ZKP, one can check that $C_y$ is the value
initially committed to, and that the input $x$ and the output $z$
are consistent. We model it using symbols $\ZK/7$, $\verZK/1$, $\Pub/1$
and equations:
\begin{align*}
    zkp & = \ZK(\langle C_x,C_y,C_z \rangle,x,y,z,r_x,r_y,r_z),
    \\
    \Pub(zkp) & = \langle C_x, C_y, C_z \rangle,
    \\
    \verZK(zkp) & = \true
\end{align*}
with 
$C_x = \commit(x,r_x)$,
$C_y = \commit(y,r_y)$,
$C_z = \commit(z,r_z)$,
and
$z=f(x,y)$.

The original protocol was implemented with hash functions and
Zero-Knowledge Succinct Non-interactive Arguments of Knowledge
(ZK-SNARKs) for performance.
%
Kroll's preliminary analysis~\cite[Section~5.2.2]{krollphd} was
informal and only considered holding the authority accountable.
%
Later analysis discovered
that any subject can falsely accuse the authority $A$ of
misbehavior~\cite{cryptoeprint:2018:127}.
%
Obviously, such a claim would subvert the trust into the system and
hence render the accountability mechanism useless in practice. 
%
Consequently, we extended the protocol with a message authentication
mechanism based on digital signatures so that $A$ and $S_i$ prove
their identity and protect themselves from false accusations, as well
as $C_{x'}$, which is a second commitment on $x$ generated by $S$
instead of $A$.

This commitment (along with $S$'es signature) serves as a witness
that
the input which $A$ claims to have received is indeed the one $S$ has sent,
without revealing $x$ to the public.
%
It is also possible to avoid maintaining both $C_{x}$ (chosen by $A$)
and $C_{x'}$ (chosen by $S$) if we allow $S$ to chose $C_{x}$, i.e.,
the commitment to $x$ in the public part of the ZKP, similar to how
the commitment to $y$ has to match the commitment sent out at the
beginning of the protocol. 
%
This is structurally closer to Kroll's original proposal, however, it
requires a slightly different proof system. We therefore modelled and
verified both fixes, but present only one here.

On the other hand, we simplified Kroll's protocol by removing
randomness generation for $f$, which was implemented using verifiable
random functions. We outline in Section~\ref{sec:concl} how this
feature calls for a definition of accountability in the computational
setting.

We model this protocol as an accountability process with three
subprocesses $A$, $S$ and
a judging procedure $J$ (see
Figure~\ref{fig:accountable-algorithms-protocol}
and~\ref{fig:accountable-algorithms-protocol-judging-procedure}).
%
This judging procedure essentially determines
the verdict by inspecting the log and a claim output by $S$. 
%
For brevity, we introduce a symbol $\mathfun{eq}/2$ with equation
$\mathfun{eq}(x,x)=\true$ and predicates $\mathfun{and3}$ and
$\mathfun{and4}$ which evaluate to true if all three or four terms
equal the constant $\true$.
%
We also use syntactic sugar $\mathsf{let}~v = t~\mathsf{in}~P$
to denote the literal substitution of $v$ by $t$ in $P$.

\begin{figure}[t]%{{{fig
\centering
\begin{lstlisting}
J$\defeq$ let res     = <'2', z, rz, rx>
      claim   = <'3', x, z, res, sig_res, rxp>
      sig_cxp = fst(log)  // log is <sig_cxp, zkp, Cxp>;
      zkp     = fst(snd(log))
      CxpL    = snd(snd(log))
      Cx      = fst(Pub(zkp))
      Cy      = fst(snd(Pub(zkp)))
      Cz      = snd(snd(Pub(zkp)))
in
in (<claim, sig_claim>);
if verify(sig_claim, claim, pk(sk('S'))) = true() then
  lookup <'A','Final'> as y in 
  event Final();
  lookup <'A','Init'> as CyL in
  event Comm(CyL);
  lookup <'A','Log','S'> as log in
  // first check validity of the log by itself,
  if and3(verZK(zkp), eq(CyL, Cy), //produced by A
    verify(sig_cxp,CxpL,pk(sk('S')))) //verified by A 
  then 
      if and3(verify(sig_res,res,pk(sk('A'))), // honest S verifies this
              verCom(CxpL,rxp), // produced by S
              eq(x, open(CxpL,rxp)))) // both signed by S 
      then // We now believe S is honest and its claim valid
        if and4(verCom(Cx,rx), verCom(Cz,rz),
                eq(x, open(Cx, rx)),eq(z, open(Cz, rz)))
        then 
          event Control('0','1');event HonestS();
          event HonestA();event Verified(claim)
        else 
          if oracle(x,Cy,z)=true() then // see below.
            event Control('0','2');event HonestS();
            event HonestA(); event Verified(claim)
          else 
            event Control('0','3');event HonestS();
            event DisHonestA(); event Verified(claim)
      else  // A's log is ok, but S is definitely cheating
        if oracle(x,Cy,z)=true() then
          event Control('0','4');event HonestS();
          event HonestA(); event Verified(claim))
        else 
          event Control('0','5');event DisHonestS();  
          event HonestA();event Verified(claim)
  else (// A is dishonest and produced bad log
    if oracle(x,CyL,z)=true() then
      event Control('0','6');event HonestS();
      event HonestA();event Verified(claim)
    else
      event Control('0','7');event DisHonestA();
      event DisHonestS();
      // S checks log before submitting claim$\rightarrow$ S dishonest
      event Verified(claim))
\end{lstlisting}
\caption{Accountable algorithms protocol: judging procedure.}
\label{fig:accountable-algorithms-protocol-judging-procedure}
\end{figure} %}}}

The verdict function is a trivial conversion of the events emitted by
the judging procedure $J$, which inspects the log and evaluates the
claim for consistency (see
Figure~\ref{fig:accountable-algorithms-protocol-judging-procedure}).
%
We decided for this approach in order to ensure that the judgement can
be made by the public, and to provide an algorithmic description on
how to do so, since a verdict function can easily be written to rely on
information that is not available or not computable.
%
$J$ is technically a trusted party in the sense that it is always honest.
However, J is not involved in the protocol and the fact can be
computed after the fact by anyone who receives the claim, e.g.,
a newspaper, an oversight body, or the general public.
%
A dishonest $J$ merely means that the verdict function is computed
incorrectly, in which case we cannot, and should not, make any guarantees.
%
The verdict function maps traces in which
$\DishonestA$ and $\DishonestS$ appear to be $\set{\set{A,S}}$,
and traces with
$\DishonestA$ and $\HonestS$ to be $\set{\set{A}}$.
%
It provides the protocol with accountability for the following property
$\varphi$:
\begin{align*}
    \forall t,x,z,r,\sig_r,r_{x'}. & 
    \Verified(\langle t,x,z,r,\sig_r,r_{x'} \rangle)@k 
    \\
     \implies \exists j,i,y,r_y. &
    \Final()@i \land \CommEv(\commit(y,r_y))@j 
    \\
    & \land z = f(x,y) \land
    i<j<k.
\end{align*}

This property guarantees that any claim considered by the judging
procedure is correctly computed w.r.t. $f$ and the initial commitment
to $y$. Note that a violation requires a $\Verified$-event, which $J$
only emits if, and only if, the first conditional and the two
subsequent lookups are successful.
%
The conditional formulates the requirement of a claim to be signed by
$S$, the two lookups require $A$ to indicate the
protocol is finished and to have produced an Init entry, in order to
ensure that the claim is only filed after the protocol has finished.

The judging procedure needs to rely on an external oracle to determine
whether a violation actually took place. This is a restriction, as it
requires any party making a judgement to have access to such an
oracle.
%
We need this for the following reason: accountability implies
verifiability, hence, even if the logs have been tampered with, and
they do not contain usable information, the verdict function needs to
nevertheless output the empty verdict if $z=f(x,y)$. For example, if $C_y$ in the
log does not match $x'$ and $z$ in claim, i.e., $z\neq f(x',\open(C_y,r_y))$,
but the logged $C_x$ is a commitment to
a different $x$, it could well be the case that $z=f(x,y)$.
%
Figuratively speaking, the adversary tries to trick us into thinking
something went wrong.
%
We represent the oracle as a function symbol $\oracle/3$ with equation
$\oracle(x,\commit(y,ry),f(x,y))=\true$, and restrain ourselves to
only use this function in the judging procedure.

The judging procedure is instructive in the constraints it
puts on the parties. Broadly speaking, they have to assist $J$
in holding the opposite party accountable by validating
incoming messages. E.g., if $A$ manipulates the log by
providing an invalid ZKP, $S$ terminates, and $\varphi$ is trivially
true.
%
This ensures that $J$ can count on the validity of the log unless $S$
is dishonest. On the other hand, $A$ can now stall the process.
%
From a protocol design perspective, this raises the following
challenges:
\begin{inparaenum}[\itshape 1.\upshape]
    \item Are there guiding principles for the judging procedure? (Our
        design involved a lot or trial and error, which is only
        a viable strategy due to the tool support we have.)
    \item Is it possible to achieve accountability for
        timeliness, i.e., the property that the protocol eventually
        finishes~\cite{BaDrKr-2016-liveness}?
    \item Can we do
        without oracle access in the judging procedure?
\end{inparaenum}


==> def-trans.tex <==
$$
\begin{array}{r c l}
    \sem{0, p,\tilde x}\underscorethingy & = & \theactualrule{
   [\state_p(\tilde x)  ] \msrewrite{~} []
   } \\
   % ,\\
   % && \phantom{\{}
   % [\semistate_{p}(\tilde x) ] \msrewrite{~} []
   % }
% \\

  \sem{P \mid Q, p, \tilde x}\underscorethingy & = & \theactualrule{
                                                     [\state_p(\tilde
                                                     x)]
                                                     \msrewrite{\ProgFrom_p,\ProgTo_{p\cdot 1}, \ProgTo_{p\cdot 2}}
    [\state_{p\cdot 1}(\tilde x_p), \state_{p\cdot 2}(\tilde x_p)]} \\
  & & \cup
  \sem{P, p\cdot 1, \tilde x_p}\underscorethingy\cup \sem{Q, p\cdot 2,
    \tilde x_p}\underscorethingy\\

  \sem{P + Q, p, \tilde x}\underscorethingy & = & 
\sem{P, p\cdot 1, \tilde x}\underscorethingy \left\{ ^{\state_p(\tilde x)} / _{\state_{p\cdot1}(\tilde x)} \right\} 
   \cup \sem{Q, p\cdot 2, \tilde x}\underscorethingy \left\{ ^{\state_p(\tilde x)} / _{\state_{p\cdot2}(\tilde x)} \right\}  \\


   \sem{! P, p, \tilde x}\underscorethingy & = & \theactualrule{
   [\state_p(\tilde x)  ] \msrewrite{\ProgTo_{p\cdot 1}} [!\semistate_{p}(\tilde x)],\\
   && \phantom{\{}
   [!\semistate_{p}(\tilde x)] \msrewrite{~} [\state_{p\cdot 1}(\tilde x)]
   }
    \cup \sem{P, p\cdot 1, \tilde x}\underscorethingy\\

   \sem{\nu a;P, p, \tilde x}\underscorethingy & = & \theactualrule{[\state_p(\tilde x),
  \Fr(n_a:\freshsort)]
  \msrewrite{\ProgFrom_p,\ProgTo_{p\cdot 1},\ProtoNonce(n_a:\freshsort)} \\
  && \phantom{\{} [\state_{p\cdot 1}(\tilde x,n_a:\freshsort)]}  \cup \sem{P, p\cdot 1, (\tilde
    x, n_a:\freshsort)}\underscorethingy  \\

  \sem{\pout(\resc, m);P, p, \tilde x}\underscorethingy & = &  
\theactualrule{
    [\state_p(\tilde x),\MIDSender(\mathit{mid}) ]
\msrewrite{\ProgFrom_p,\ProgTo_{p\cdot 1},\Send(\mathit{mid},m)} \\
&&\phantom{\{} 
[\state_{p\cdot 1}(\tilde x,\mathit{mid}), \Out(m)]}
 \cup \sem{P, p\cdot 1, \tilde x}\underscorethingy\\


  \sem{\pin(\resc,m);P, p, \tilde x}\underscorethingy & = & 
 \theactualrule{
       [\state_p(\tilde x),\In(m),\Fr_p,\MIDReceiver(\mathit{mid})]
       \msrewrite{\ProgTo_{p\cdot
       1},\Receive(\mathit{mid},m),\ChannelInEvent(m)}\\
       && \qquad
          [\state_{p\cdot 1}(\tilde x_p \cup \vars(m))]  
          }\\
   & & \cup \sem{P, p\cdot
     1, \tilde x \cup \vars(m)}\underscorethingy\\


  \sem{\pout(\pubc,N);P, p, \tilde x}\underscorethingy & = &  
     \theactualrule{
         [\state_p(\tilde x), \In(\pubc)]
     \msrewrite{\ProgFrom_p,\ProgTo_{p\cdot 1},\ChannelInEvent(\pubc) }  [\state_{p\cdot 1}(\tilde x), \Out(N)]}\\
& &  \cup \sem{P, p\cdot 1, \tilde x_p}\underscorethingy\\


  \sem{\pin(\pubc,m);P, p, \tilde x}\underscorethingy & = & 
\theactualrule{
 [\state_p(\tilde x), \In(\pair \pubc m ), \Fr_p ]
 \msrewrite{\ProgTo_{p\cdot 1},\ChannelInEvent(\pair \pubc m) }\\
  && \qquad [\state_{p\cdot 1}(\tilde x \cup \vars(m)) ]
       }\\
  & & \cup \sem{P, p\cdot
    1, \tilde x \cup \vars(m)}\underscorethingy\\


  \begin{array}{r}
    \llbracket\mbox{if }\pr(M_1,\ldots,M_k)\quad\\
      \mbox{ then }P \mbox{ else } Q ,
      p, \tilde x\rrbracket\underscorethingy 
  \end{array}
  & = &
  \begin{array}{l}
  \theactualrule{
    [\state_p(\tilde x)]
    \msrewrite{\ProgFrom_p,\ProgTo_{p\cdot 1},\mbox{Pred}_{\pr}(M_1,\ldots,M_k)} [\state_{p\cdot 1}(\tilde
    x)],\\
    \phantom{\{}
    [\state_p(\tilde x)]
    \msrewrite{\ProgFrom_p,\ProgTo_{p\cdot 1},\mbox{Pred_not}_{\pr}(M_1,\ldots,M_k)} [\state_{p\cdot
      2}(\tilde x)] }
   \end{array}\\
   & & \cup \sem{P, p\cdot 2, \tilde x}\underscorethingy \cup \sem{Q, p\cdot 2, \tilde x}\underscorethingy\\

  \sem{\mbox{event }F;P, p, \tilde x}\underscorethingy & = & 
\theactualrule{
 [\state_p(\tilde x)]
\msrewrite{\ProgFrom_p,\ProgTo_{p\cdot 1},\Event(),F}
  [\state_{p\cdot 1}(\tilde x)] } \cup \sem{P, p\cdot 1,\tilde x}\underscorethingy\\

  \sem{\mbox{insert } s, t ; P, p, \tilde x}\underscorethingy & = & 
\theactualrule{
 [\state_p(\tilde x)]
 \msrewrite{\ProgFrom_p,\ProgTo_{p\cdot 1},\mathrm{Insert}(s,t)}
  [\state_{p\cdot 1}(\tilde x)] } \cup \sem{P, p\cdot 1, \tilde x}\underscorethingy\\

  \sem{\mbox{delete } s; P, p, \tilde x}\underscorethingy & = & 
\theactualrule{
[\state_p(\tilde x)]
  \msrewrite{\ProgFrom_p,\ProgTo_{p\cdot 1},\mathrm{Delete}(s)}
  [\state_{p\cdot 1}(\tilde x)] } \cup \sem{P, p\cdot 1, \tilde x}\underscorethingy\\

  \begin{array}{r}
    \llbracket
     \mbox{lookup } M\mbox{ as }v \mbox{ in } P
    \\
 \mbox{ else } Q ,
      p, \tilde x\rrbracket\underscorethingy 
  \end{array}
  
  & = & 
\theactualrule{
 [\state_p(\tilde x)]
  \msrewrite{\ProgFrom_p,\ProgTo_{p\cdot 1},\mathrm{IsIn}(M,v)}
  [\state_{p\cdot 1}(\tilde M,v)],\\
  && \phantom{\{} [\state_p(\tilde x)]
     \msrewrite{\ProgFrom_p,\ProgTo_{p\cdot 2},\mathrm{IsNotSet}(M)}
  [\state_{p\cdot 2}(\tilde x)]} \\
  && \cup \sem{P, p\cdot 1, (\tilde x,v)}\underscorethingy \cup \sem{Q, p\cdot 2, \tilde x}\underscorethingy\\ 
  
  \sem{\mbox{lock}^l~s; P, p, \tilde x}\underscorethingy & = & 
\theactualrule{
    [\state_p(\tilde x),\mathrm{Fr}(\mathrm{lock}_l)]
  \msrewrite{\ProgFrom_p,\ProgTo_{p\cdot 1},\mathrm{Lock}(\mathit{lock}_l,s)}
  [\state_{p\cdot 1}(\tilde x,\mathit{lock}_l)] }\\
& & \cup \sem{P, p\cdot 1, \tilde x}\underscorethingy
  \\ 

  \sem{\mbox{unlock}^l~s; P, p, \tilde x}\underscorethingy & = & 
\theactualrule{
[\state_p(\tilde x)]
  \msrewrite{\ProgFrom_p,\ProgTo_{p\cdot 1},\mathrm{Unlock}(\mathit{lock}_l,s)}
  [\state_{p\cdot 1}(\tilde x)]}  \cup \sem{P, p\cdot 1, \tilde x}\underscorethingy
  % \\
  % \sem{\text{$[ l \msrewrite a r ]; P$},p,\tilde x}\underscorethingy & = &
  % \theactualrule{
  %   [\state_p(\tilde x), l] \msrewrite {\Event(),a} [r,\state_{p \cdot 1}(\tilde x\cup
  %   \vars(l))] }\\
  % & & \cup \sem{P, p\cdot 1, \tilde x\cup \vars(l)} 
\end{array}
$$

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "fairexchange"
%%% End: 


==> fig-semantics-reliable.tex <==
   \small 
  \newlength{\mylinespace}
  \setlength{\mylinespace}{1mm}
  {\bf Standard operations:}
  $$
  % \hspace{-3cm} 
  \begin{array}{rcl}
    (\Names, \StoreA,  \Processes \mcup \{0\}, \Subst, \ActiveLocks, \Undelivered) 
    & \longrightarrow_i &  (\Names, \StoreA,  \Processes , \Subst, \ActiveLocks, \Undelivered) \\[\mylinespace]
    (\Names, \StoreA,  \Processes \mcup \{P|Q\}, \Subst, \ActiveLocks, \Undelivered) 
    &\longrightarrow_i&
    (\Names, \StoreA,  \Processes \mcup \{P,Q\}, \Subst, \ActiveLocks, \Undelivered) 
    \\[\mylinespace]
    (\Names, \StoreA,  \Processes \mcup \{P+Q\}, \Subst, \ActiveLocks, \Undelivered) 
    &\trans{A}_i&
    (\Names', \StoreA',  \Processes', \Subst', \ActiveLocks', \Undelivered') 
    \\[\mylinespace]
    \multicolumn{3}{r}{\text{if  }
        (\Names, \StoreA,  \Processes \mcup \{P\}, \Subst, \ActiveLocks, \Undelivered) 
        \trans{ A }_i
        (\Names', \StoreA',  \Processes', \Subst', \ActiveLocks', \Undelivered') 
        \text{ or }
        (\Names, \StoreA,  \Processes \mcup \{Q\}, \Subst, \ActiveLocks, \Undelivered) 
        \trans{ A }_i
        (\Names', \StoreA',  \Processes', \Subst', \ActiveLocks', \Undelivered') 
    }
    \\[\mylinespace]
    \multicolumn{3}{r}{\text{where $\Processes'=\Processes$ or 
      $\Processes' = \Processes \mcup \mset{P'}$ for some $P'\neq P$}
    }
    \\[\mylinespace]
    (\Names, \StoreA,  \Processes \mcup \{!P\}, \Subst, \ActiveLocks, \Undelivered) 
    &\longrightarrow_i& 
    (\Names, \StoreA,  \Processes \mcup \{!P, P\}, \Subst, \ActiveLocks, \Undelivered) 
    \\[\mylinespace]
    (\Names, \StoreA,  \Processes \mcup \{\nu a;P\}, \Subst, \ActiveLocks, \Undelivered) 
    &\longrightarrow_i&
    (\Names\cup\{a'\}, \StoreA,  \Processes \mcup \{P\{^{a'}/_{a}\}
    \}, \Subst, \ActiveLocks, \Undelivered) \\
    \multicolumn{3}{r}{\text{if $a'$ is fresh}}
    \\[\mylinespace]
    (\Names, \StoreA,  \Processes, \Subst, \ActiveLocks, \Undelivered) 
    &\trans{K(M)}_i& 
    (\Names, \StoreA,  \Processes, \Subst, \ActiveLocks, \Undelivered) \quad
    {\text{if $\nu \Names.\Subst \vdash M$}}
    \\[\mylinespace]
    % resilient out
    (\Names, \StoreA,  \Processes \mcup \{\pout(\resc,N);P\},\Subst, \ActiveLocks, \Undelivered) 
    &\trans{~}_i&
    (\Names, \StoreA,  \Processes \mcup \{P\},\Subst\cup \{^N / _x\}, \ActiveLocks, \Undelivered \mcup \mset{ N} ) 
    \\
    \multicolumn{3}{r}{\text{if
      $x$ is fresh}}
    \\[\mylinespace]
    (\Names, \StoreA,  \Processes \mcup \{\pin(\resc,N);P\},\Subst, \ActiveLocks, \Undelivered) 
    &\trans{K({N\tau})}_i&
    (\Names, \StoreA,  \Processes \mcup \{P\tau \},\Subst, \ActiveLocks, \Undelivered)  
    \\
    \multicolumn{3}{r} {\text{if }\exists \tau.\ \tau\text{ is
            grounding for } N,  \nu \Names.\Subst\vdash N\tau}
    \\[\mylinespace]
    % resilient in -- correct data
    (\Names, \StoreA,  \Processes \mcup \{\pin(\resc,N);P\},\Subst, \ActiveLocks, \Undelivered) 
    &\trans{K({N\tau})}_i&
    (\Names, \StoreA,  \Processes \mcup \{P\tau \},\Subst, \ActiveLocks, \Undelivered \msetminus \mset{ {N'}})  
    \\
    \multicolumn{3}{r} {\text{if }\exists N', \tau.\ N'\in\Undelivered, \tau\text{ is
            grounding for } N,  N\tau =_E N' }
    \\[\mylinespace]
    % normal out
    (\Names, \StoreA,  \Processes \mcup \{\pout(\pubc,N);P\},\Subst, \ActiveLocks, \Undelivered) 
    &\trans{K(\pubc)}_i&
    (\Names, \StoreA,  \Processes \mcup \{P\},\Subst\cup \{^N / _x\}, \ActiveLocks, \Undelivered ) 
    \\
    \multicolumn{3}{r}{\text{if
$x$ is fresh }} % and $\nu \Names. \Subst\vdash M$}}
    \\[\mylinespace]
    (\Names, \StoreA,  \Processes \mcup \{\pin(\pubc,N);P\},\Subst, \ActiveLocks, \Undelivered) 
    &\trans{K(\pair{\pubc}{N\tau})}_i&
    (\Names, \StoreA,  \Processes \mcup \{P\tau \},\Subst, \ActiveLocks, \Undelivered)  
    \\
    \multicolumn{3}{r} {\text{if }\exists \tau.\ \tau\text{ is
            grounding for } N, \nu \Names.\Subst\vdash N\tau}
    \\[\mylinespace]
    % \multicolumn{1}{l}{(\Names, \StoreA, }
    % \\
    % \quad\quad
    % (\Names, \StoreA,  \Processes \mcup \{\pout(\pubc,N);P, \pin(\pubc,N');Q\},\Subst, \ActiveLocks, \Undelivered) 
    % &\longrightarrow_i&
    % (\Names, \StoreA,  \Processes \cup \{P, Q \tau \},\Subst, \ActiveLocks, \Undelivered)  
    % \\
    % \multicolumn{3}{r}{\text{if $\exists \tau.$ $N =_E N'\tau$ and $\tau$ grounding for $N'$}}
    \\[\mylinespace]
    (\Names, \StoreA,  \Processes \cup \{\text{if $\pr(M_1,\ldots,M_n)$ then $P$ else $Q$}\},\Subst, \ActiveLocks, \Undelivered) 
    &\longrightarrow_i&
    (\Names, \StoreA,  \Processes \cup \{P\}, \Subst, \ActiveLocks, \Undelivered) \\
    && \quad\text{if $\phi_\pr\{^{M_1} / _{x_1},\ldots, ^{M_n} / _{x_n}\}$ is satisfied}
    \\[\mylinespace]
    (\Names, \StoreA,  \Processes \cup \{\text{if $\pr(M_1,\ldots,M_n)$ then $P$ else $Q$}\}, \Subst, \ActiveLocks, \Undelivered) 
    &\longrightarrow_i& 
    (\Names, \StoreA,  \Processes \cup \{Q\}, \Subst, \ActiveLocks, \Undelivered)  \\
    && \quad\text{if $\phi_\pr\{^{M_1} / _{x_1},\ldots, ^{M_n} / _{x_n}\}$ is not satisfied}
    \\[\mylinespace]
    (\Names, \StoreA,  \Processes \cup \{\text{event($F$); $P$}\}, \Subst, \ActiveLocks, \Undelivered) 
    &\stackrel{F}{\longrightarrow_i}&
    (\Names, \StoreA,  \Processes \cup \{P\}, \Subst, \ActiveLocks, \Undelivered)
  \end{array}
$$
{\bf Operations on global state:}
$$
\begin{array}{rcl}
  (\Names, \StoreA,  \Processes \mcup \{\text{insert $M,N$; $P$}\},
  \Subst, \ActiveLocks, \Undelivered) 
  &\longrightarrow_i& 
  (\Names, \StoreA[M\mapsto N ],  \Processes \mcup \{P\},  \Subst,
  \ActiveLocks, \Undelivered)  
  \\[\mylinespace]
  (\Names, \StoreA,  \Processes \mcup \{\text{delete $M$; $P$}\},
  \Subst, \ActiveLocks, \Undelivered) 
  &\longrightarrow_i&
  (\Names, \StoreA[M \mapsto \bot],  \Processes \mcup \{P\},  \Subst,
  \ActiveLocks, \Undelivered)  % \\
  % \multicolumn{3}{r}{\text{ where }\StoreA'(x) = \begin{cases}
  %   \StoreA(x)  & \text{if  $x\neq_E M$} \\
  %   \bot  & \text{otherwise}
  % \end{cases}}
  \\[\mylinespace]
  (\Names, \StoreA,  \Processes \mcup \{\text{lookup $M$ as $x$ in $P$
    else $Q$ }\},  \Subst, \ActiveLocks, \Undelivered) 
  &\longrightarrow_i&
  (\Names, \StoreA,  \Processes \mcup \{ P\{V/x\}\},  \Subst,
  \ActiveLocks, \Undelivered)\\
  \multicolumn{3}{r}{\text{if $\StoreA(M)=_E V$ is defined}} \\[\mylinespace]
  (\Names, \StoreA,  \Processes \mcup \{\text{lookup $M$ as $x$ in $P$
    else $Q$ }\},  \Subst, \ActiveLocks, \Undelivered) 
  & \longrightarrow_i & 
  (\Names, \StoreA,  \Processes \mcup \{ Q \},  \Subst,
  \ActiveLocks, \Undelivered)\\
  \multicolumn{3}{r}{\text{if $\StoreA(M)$ is undefined}}\\[\mylinespace]

  (\Names, \StoreA,  \Processes \mcup \{\text{lock $M$; $P$}\},
  \Subst, \ActiveLocks, \Undelivered) 
  &\longrightarrow_i&
  (\Names, \StoreA,  \Processes \mcup \{P\},  \Subst,
    \ActiveLocks \cup \set{M}, \Undelivered)
    \quad\text{if $ M{\not\in}_\ET\ActiveLocks$} \\[\mylinespace]
  % unlock
  (\Names, \StoreA,  \Processes \mcup \{\text{unlock $M$; $P$}\},
  \Subst, \ActiveLocks, \Undelivered )
  &\longrightarrow_i&
  (\Names, \StoreA,  \Processes \mcup \{P\},  \Subst, \ActiveLocks
  \setminus \set{ M' \mid M'=_E M},
  \Undelivered
  )  
  \end{array}
  $$

